A linguistically-motivated evaluation methodology for unraveling model's abilities in reading comprehension tasks

We introduce an evaluation methodology for reading comprehension tasks based on the intuition that certain examples, by the virtue of their linguistic complexity, consistently yield lower scores regardless of model size or architecture. We capitalize on semantic frame annotation for characterizing this complexity, and study seven complexity factors that may account for model's difficulty. We first deploy this methodology on a carefully annotated French reading comprehension benchmark showing that two of those complexity factors are indeed good predictors of models' failure, while others are less so. We further deploy our methodology on a well studied English benchmark by using Chat-GPT as a proxy for semantic annotation. Our study reveals that fine-grained linguisticallymotivated automatic evaluation of a reading comprehension task is not only possible, but helps understand models' abilities to handle specific linguistic characteristics of input examples. It also shows that current state-of-the-art models fail with some for those characteristics which suggests that adequately handling them requires more than merely increasing model size.

==> additional_analysis.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|}
\cline{2-8}
                          & Rouge-L     & \% correct & $P(f2\mid S)$ & $P(f3\mid S)$ & $P(f4\mid S)$ & $P(f5\mid S)$ & $P(f6\mid S)$ \\ \hline
\multicolumn{1}{|c|}{S1}  & 0.80 - 0.92 & 100        & 0.35    & 0.44    & 0.26    & 0.55    & 0.53    \\ \hline
\multicolumn{1}{|c|}{S2}  & 0.54 - 0.68 & 43 - 56    & 0.38    & 0.47    & 0.32    & 0.65    & 0.61    \\ \hline
\multicolumn{1}{|c|}{all} & 0.69 - 0.82 & 71 - 82    & 0.37    & 0.46    & 0.29    & 0.59    & 0.57    \\ \hline
\end{tabular}%
}
\caption{Probability of having the $fi$ factor with \textbf{S1} the split of "easy" examples (where models agree and on the right answer), \textbf{S2} the other examples considered as "hard" and \textbf{all} on all the corpus.}
\label{tab:proba-factor}
\end{table}

Figure \ref{fig:proba-factor-agreement} shows that the probabilities of the presence of factors $f5$ and $f6$ vary the most. These factors start with a high probability in the subsets where the models disagree the most and consistently remain the most probable factors across all subsets.

\begin{figure}
 \begin{center}
  \includegraphics[width=0.5\textwidth]{images_proba_factor_agreement.pdf} 
  \caption{Probability of having the $fi$ factor by split of the example according to the number of agreement between the models}
 \label{fig:proba-factor-agreement}
 \end{center}
 \end{figure}

 \begin{figure*}[h]
 \begin{center}
  \includegraphics[width=1\textwidth]{images_natural_qa_natural_qa_difficult.pdf} 
  \caption{Models F1 score on 3 partitions of the difficult subset of the evaluation corpus according to $f6$, "*" denotes a significant score difference}
 \label{fig:score_natural_qa_difficult}
 \end{center}
 \end{figure*}

 \begin{figure*}[h]
 \begin{center}
  \includegraphics[width=1.2\textwidth]{images_natural_qa_natural_qa_all.pdf} 
  \caption{Models F1 score on 3 partitions of the evaluation corpus according to $f6$, "*" denotes a significant score difference}
 \label{fig:score_natural_qa_all}
 \end{center}
 \end{figure*}


\begin{figure*}[h!]
 \begin{center}
  \includegraphics[width=1\textwidth]{images_natural_qa_natural_qa_fe_all.pdf} 
  \caption{Models F1 score on 3 partitions of the evaluation corpus according to $f5$, "*" denotes a significant score difference}
 \label{fig:score_natural_qa_fe_all}
 \end{center}
 \end{figure*}


\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|cc|}
\hline
                                  & \multicolumn{2}{c|}{Factors}                   \\ \hline
models/factors                    & \multicolumn{1}{c|}{f5}          & f6          \\ \hline
size of Ef (\%)                   & \multicolumn{1}{c|}{80\%}        & 52\%        \\ \hline
google\_text-bison@001            & \multicolumn{1}{c|}{0}           & -2          \\ \hline
qwen\_qwen1.5-32b                 & \multicolumn{1}{c|}{-3}          & \textbf{-6} \\ \hline
meta\_llama-3-70b                 & \multicolumn{1}{c|}{-4}          & \textbf{-6} \\ \hline
mistralai\_mixtral-8x7b-32kseqlen & \multicolumn{1}{c|}{\textbf{-9}} & \textbf{-8} \\ \hline
meta\_llama-3-8b                  & \multicolumn{1}{c|}{-5}          & \textbf{-8} \\ \hline
google\_gemma-7b                  & \multicolumn{1}{c|}{-4}          & -4          \\ \hline
meta\_llama-2-7b                  & \multicolumn{1}{c|}{-8}          & -5          \\ \hline
mistralai\_mistral-large-2402     & \multicolumn{1}{c|}{1}           & \textbf{-6} \\ \hline
\end{tabular}%
}
\caption{Hard subset of naturalQA}
\label{tab:complex-naturalQA-hard}
\end{table}

\begin{figure*}[h]
 \begin{center}
  \includegraphics[width=1\textwidth]{images_natural_qa_natural_qa_fe_entropy_hard.pdf} 
  \caption{Models F1 score on 3 partitions of the difficult subset of the evaluation corpus according to combinations of complexity factors $f5$ and $f6$}
 \label{fig:natural_qa_fe_entropy_hard}
 \end{center}
 \end{figure*}


==> corpus_production.tex <==
\subsection{A semantically controlled reading comprehension corpus}
\label{sec:corpus}

In this study, we use the publicly available \calor corpus, which contains documents semantically annotated with the Berkeley Framenet semantic model. This corpus includes French texts from Wikipedia and ClioTexte, a collection of historical documents used in French schools. The texts cover three main themes: the First World War, archaeology, and antiquity.

The semantic annotation of this corpus consists of Semantic Frames that describe prototypical situations (e.g., decide, lose, attack, defeat). First, the trigger word of the Frame, called the Lexical Unit (LU), is identified, followed by the specification of the arguments, known as Frame Elements (FE). 

In \cite{bechet2019calor}, the \calor corpus was enriched with a set of semantically controlled \textit{questions/answers} examples with the following method: a \textit{Frame} $F$ and one of its \textit{Frame Element} $E$ are randomly selected within a sentence; a human annotator is then presented with these elements and tasked with generating a question whose answer is $E$, relying on the semantic relationship between $F$ and $E$. The other \textit{FEs} present in the sentence constitute the context $C$ of the question and can be employed to provide additional context to the question. By varying $F$, $E$, and $C$ for the same sentence, we can generate a set of questions for which we have the answers, along with their semantic class (the type of \textit{FE}).

In cases where answers necessitate resolving coreferences, the coreference chain leading back to the sought answer is also annotated. 
Through this methodology, a corpus comprises \textit{1785} questions has been obtained, derived from a total of 54 semantic frames.


==> mrqa_task.tex <==
\section{Application to a Machine Reading Comprehension task}



The document-based question-answering task has been extensively studied since the rise of deep neural network-based models, facilitated by large evaluation corpora such as SQuAD~\cite{D16-1264} and MultiRC~\cite{khashabi2018looking}, part of the SuperGLUE benchmark~\cite{wang2019superglue}. Transformer-based language models consistently outperform humans on these leaderboards\footnote{\url{https://rajpurkar.github.io/SQuAD-explorer}, \url{https://super.gluebenchmark.com/leaderboard}}, highlighting the challenge of evaluating models due to the subjective nature of answer generation and their ability to replicate biases present in training data.

Despite its limitations, this task offers advantages: (1) it allows comparing classification and generation models, both achieving comparable performance despite the smaller and simpler nature of classification models; (2) the task can be partially formalized using linguistic models to explain syntactic and semantic connections between questions and answers. This is a notable advantage from purely generative tasks like automatic summarization or translation, which pose greater challenges in linguistic formalization.



\input{corpus_production}
\input{qa_models}
\input{complexity_factors}


==> natural_qa.tex <==
\section{Application to NaturalQA}

\begin{table}[]
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{|cc|cc|}
\hline
\multicolumn{2}{|c|}{}                                  & \multicolumn{2}{c|}{Factors}            \\ \hline
\multicolumn{1}{|c|}{models/factors}             & F1   & \multicolumn{1}{c|}{f5}   & f6          \\ \hline
\multicolumn{1}{|c|}{size of ${E}_{f}$ (\%)}            &      & \multicolumn{1}{c|}{78\%} & 52\%        \\ \hline
\multicolumn{1}{|c|}{google\_text-bison@001}     & 0.81 & \multicolumn{1}{c|}{0}    & -1          \\ \hline
\multicolumn{1}{|c|}{openai\_text-davinci-003}   & 0.77 & \multicolumn{1}{c|}{-4}   & \textbf{-5} \\ \hline
\multicolumn{1}{|c|}{ROVER}  & 0.77 & \multicolumn{1}{c|}{-4}   &    -3       \\ \hline
\multicolumn{1}{|c|}{meta\_llama-3-70b}          & 0.74 & \multicolumn{1}{c|}{-3}   & \textbf{-4} \\ \hline
\multicolumn{1}{|c|}{mistralai\_mixtral-8x7b-32kseqlen} & 0.70 & \multicolumn{1}{c|}{\textbf{-6}} & \textbf{-4} \\ \hline
\multicolumn{1}{|c|}{openai\_gpt-3.5-turbo-0613} & 0.68 & \multicolumn{1}{c|}{-4}   & \textbf{-6} \\ \hline
\multicolumn{1}{|c|}{google\_gemma-7b}           & 0.66 & \multicolumn{1}{c|}{-4}   & -3          \\ \hline
\multicolumn{1}{|c|}{AlephAlpha\_luminous-extended}     & 0.61 & \multicolumn{1}{c|}{\textbf{-7}} & \textbf{-5} \\ \hline
\multicolumn{1}{|c|}{databricks\_dbrx-instruct}  & 0.55 & \multicolumn{1}{c|}{-2}   & 0           \\ \hline
\hline
\rowcolor{lightgray} \multicolumn{1}{|c|}{ROVER}  & 0.77 & \multicolumn{1}{c|}{-4}   &    -3       \\ \hline
\end{tabular}%
}
\caption{Validation results for $f5$ and $f6$ across models on naturalQA.
'\textit{Size}' indicates proportions of partitions $E_{f}$ relative to the total corpus.}
\label{tab:complex-naturalQA}
\end{table}

 \begin{figure*}[]
 \begin{center}
  \includegraphics[width=1\textwidth]{images_natural_qa_natural_qa_fe_entropy_all.pdf} 
  \caption{Models F1 score on 3 partitions of the evaluation corpus according to combinations of complexity factors $f5$ and $f6$}
 \label{fig:natural_qa_fe_entropy_all}
 \end{center}
 \end{figure*}


To check the transferability of our two main complexity factors ($f5$ and $f6$) to other datasets and languages, we used the subset of NaturalQA \cite{kwiatkowski2019natural} and the predictions of 48 models made available by HELM \cite{liang2023holistic} on their \textit{natural\_qa\_openbook\_longans}\footnote{\url{https://crfm.stanford.edu/helm/lite/latest/\#/groups/natural_qa_openbook_longans}} scenario. This consists of 1,000 examples of NaturalQA's evaluation distribution, made up of a question, a "short" answer and the context, in this case the corresponding "long" answer in NaturalQA (often equivalent to a paragraph). Table~\ref{tab:complex-naturalQA} presents an overview of the results for 8 models and ROVER applied in the same way, selected to represent the full range of mean F1 scores across the 48 models.

\paragraph{Applying $f6$ to NaturalQA.} For this dataset, lacking an automatic Frame analysis, we used a proxy method: we compiled potential triggers from Berkeley FrameNet frames and checked their presence in the questions. Each question provided a list of triggers and their corresponding frames. Using a custom prompt\footnote{see Appendix~\ref{appendix:NaturalQA}}, we employed GPT-3.5 to determine the most appropriate pair for each question.

Out of 1000 examples, 18 had no extractable triggers and were discarded. On the generated Frames by GPT-3.5, 35 were unknown from our Frame dictionnary and were also discarded. We then assessed our $f6$ factor by calculating the median entropy across all Berkeley FrameNet frames.

Examples with entropy above the median generally scored below the overall average, while those below it scored above. Across all models, the average difference in performance between these subsets was -3.17 (± 1.82) F1 points, impacting 12 models significantly.



 


 \paragraph{Applying $f5$ to NaturalQA.} Since NaturalQA questions often do not consist only of text paragraphs and our Frames are derived from these questions, we automatically extract Frame Elements based on previously predicted Frames to proxy $f5$. Using an empirically developed prompt (see Appendix~\ref{appendix:NaturalQA} ), we extracted Frame Elements for 937 examples where Frames were successfully predicted out of 961 attempts (24 were discarded due to output issues).

We then categorize these examples based on our $f5$ factor : those with more than 2 are considered easier, while those with 2 or fewer are considered more challenging. Typically, examples with more than 2 Frame Elements score above the overall average, while those with 2 or fewer score below. However, on average, this difference is smaller and statistically significant for fewer models compared to $f6$. On average, across all models, the difference in performance between these subsets is -3.84 (± 2.44) F1 points. This may be due from NaturalQA questions being simpler and containing fewer Frame Elements compared to our original corpus, increasing the proportion of challenging examples from 60\% to 78\%.



 




==> qa_models.tex <==
\subsection{Language models for reading comprehension}

In this study, we compare seven pre-trained language models on our text-based QA task using the \calor corpus. Among these models, one is a classification model based on a BERT architecture developed for the French language, CamemBERT \cite{devlin-etal-2019-bert, martin2020camembert}. Three models are multilingual generative models based on \textbf{T5} (T5-LARGE, FLAN-T5-LARGE \cite{wei2021finetuned}, MT5-LARGE \cite{xue2020mt5}), and three models are current Large Language Models (LLMs): LLAMA2 \cite{touvron2023llama}, Mixtral 8x7B \cite{jiang2024mixtral} and chatGPT-3.5\footnote{API from \url{https://chat.openai.com}}.

All these pre-trained models, except GPT3.5 and Mixtral 8x7B, have been adapted to our QA task using the French corpus FQuAD \cite{dhoffschmidt-etal-2020-fquad}. This corpus, constructed similarly to SQuAD \cite{D16-1264}, contains questions based on French Wikipedia documents. It's worth noting that while most texts in the \calor corpus are also sourced from Wikipedia, \calor is notably more challenging than FQuAD. This difference arises because the texts in \calor are specialized, and the annotated responses are significantly longer, corresponding to the Frame Elements of our semantic annotations.

The formats of the FQuAD and $\calor$ corpora have been unified to allow the evaluation of a system adapted with FQuAD directly on \calor.



We fine-tuned CamemBERT and T5 models on FQuAD for 2 epochs, applied the \textit{Low-Rank Adaptation} (LoRA) method \cite{hu2021lora} to LLAMA2, and used one-shot and two-shot prompting approaches for GPT-3.5 and Mixtral 8x7B, respectively. This involved specifying to the model the requirement for an extraction of the original document with one example of input/output in the expected format.

Evaluation of these six models on the \calor corpus employed two types of metrics: automatic and human. Automatic metrics included the \textit{ROUGE-L} score from the ROUGE toolkit\footnote{We used the Google Research implementation available \href{https://github.com/google-research/google-research/tree/master/rouge}{here}, with the stemmer and CamemBERT-base tokenizer.} \cite{lin-2004-rouge}, measuring similarity between the extractive reference answer and system output. For human evaluation, we conducted manual annotation of all system outputs. Annotators assessed triplets comprising context, question, and answer, assigning labels of '\textit{correct}', '\textit{partially correct}', or '\textit{incorrect}'.

The dataset comprised 14,280 triplets, with 5,857 unique after removing duplicate answers, divided into 10 folds and evaluated by 10 human annotators. Any discrepancies between annotator labels and ground-truth were resolved through review to ensure accuracy. From this annotation, two metrics were derived:
\begin{itemize}
    \item \textit{Hscore}: Scores answers as 1 for \textit{correct}, 0.5 for \textit{partially correct}, and 0 for \textit{incorrect}.
    \item \textit{Hcorrect}: Represents the proportion of \textit{correct} answers identified by annotators for each system.
\end{itemize}


\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\rowcolor{lightgray} Model & adapt & \#param & Rouge-L & Hscore & \% Hcorrect \\ \hline
\textit{CamemBERT} & FT & 335M & 0.82 & 0.85 & 78.9 \\ \hline
\textit{T5-L} & FT & 738M &  0.81 & 0.84 &  78.0 \\ \hline
\textit{FLAN-T5-L} & FT & 783M & 0.80 & 0.85 &  79.2\\ \hline 
\textit{MT5-L}  & FT & 1.2B & 0.80 & 0.84 & 77.5 \\ \hline 
\textit{LLAMA-2}  & LoRA & 7B & 0.69 & 0.78 & 72.2 \\ \hline
\textit{Mixtral-8x7b}  & prompt & 47B & 0.80 & 0.87 & \textbf{82.6} \\ \hline
\textit{GPT 3.5} & prompt & 175B & 0.72 & \textbf{0.88} & 82.5 \\ \hline 
\rowcolor{yellow} \textit{\textbf{ROVER}} & - & - & \textbf{0.84} & \textbf{0.88} & 82.3 \\ \hline
\end{tabular}
}
\caption{Overview of the performance of the 7 models in our experiments, evaluated using Rouge-L, Hscore, and Hcorrect metrics. The final row shows the combined performance of the systems using the ROVER method."\label{tab:rouge-global}}
\end{table}

Overall, the results achieved by the various models are notably lower compared to those showcased on leaderboards of analogous tasks such as SQuAD \footnote{\url{https://rajpurkar.github.io/SQuAD-explorer}} or MultiRC in SuperGLUE \footnote{\url{https://super.gluebenchmark.com/leaderboard}}. This discrepancy can be attributed in part to the characteristics of the \calor corpus, the differences between the adaptation corpus FQuAD and the evaluation corpus \calor as discussed previously, and also to the absence of systematic model optimization through hyperparameterization.





The RougeL scores of T5-based models and CamemBERT show close alignment, while LLAMA-2 and GPT-3.5 lag significantly behind. This is due to the \calor corpus favoring extractive models, which biases RougeL metrics towards models that replicate segments without adding words.

In contrast, human evaluation favors lightly adapted generative LLMs, which enhance outputs with additional elements for clarity or explanation. These models consistently outperform others on metrics like \textit{Hscore} and \textit{Hcorrect}, highlighting the limitations of string similarity metrics in assessing generative models for abstractive tasks.

LLAMA-2 consistently underperforms in human evaluations compared to GPT-3.5 and Mixtral, possibly due to ineffective LoRA adaptation despite RougeL score monitoring. Initial assumptions about LLAMA-2's low RougeL score being attributed to its abstractive capabilities were disproven by human evaluation. Given the high cost of human annotation, using this metric to refine adaptations was impractical. Consequently, LLAMA-2 results are excluded from further study, and human metrics replace RougeL  for the remainder of our analysis.




